Weyl Covariance, and Proposals for Superconformal Prepotentials in 10D Superspaces

Proposals are made to describe the Weyl scaling transformation laws of supercovariant derivatives $\nabla{}_{\underline A}$, the torsion supertensors $T{}_{{\underline A} \, {\underline B}}{}^{{\underline C}}$, and curvature supertensors $R{}_{{\underline A} \, {\underline B}}{}_{\, \underline c} {}^{\underline d}$ in 10D superspaces. Starting from the proposal that an unconstrained supergravity prepotential for the 11D, $\mathcal{N}$ = 1 theory is described by a scalar superfield, considerations for supergravity prepotentials in the 10D theories are enumerated. We derive infinitesimal 10D superspace Weyl transformation laws and discover ten possible 10D, $\mathcal{N}$ = 1 superfield supergravity prepotentials. The first identification of all off-shell ten dimensional supergeometrical Weyl field strength tensors, constructed from respective torsions, is presented.

==> front.tex <==
%C0L0RS
%:Coloring
% Greg's colors
\definecolor{Green}  {rgb}{0.10,0.70,0.10} %  1
\definecolor{Orange} {rgb}{1.00,0.50,0.15} %  2
\definecolor{Red}    {rgb}{0.90,0.00,0.12} %  3
\definecolor{Purple} {rgb}{0.50,0.25,0.55} %  4
\definecolor{Turque} {rgb}{0.00,0.65,0.85} %  5
\definecolor{Blue}   {rgb}{0.00,0.00,1.00} %  6
\definecolor{Magenta}{rgb}{1.00,0.00,1.00} %  7
\definecolor{Gold}   {rgb}{1.00,0.75,0.25} %  8
\definecolor{Seaweed}{rgb}{0.01,0.24,0.09} %  9
\definecolor{Brown}  {rgb}{0.43,0.26,0.32} % 10
\definecolor{grey1}  {rgb}{0.20,0.20,0.20} % 11
\definecolor{grey2}  {rgb}{0.40,0.40,0.40} % 12
\definecolor{grey3}  {rgb}{0.60,0.60,0.60} % 13
\definecolor{grey4}  {rgb}{0.80,0.80,0.80} % 14
\definecolor{grey5}  {rgb}{0.90,0.90,0.90} % 1
\def\C#1#2{{\ifcase#1\or%Greg's color scheme
             \color{Green}\or \color{Orange}\or \color{Red}\or
              \color{Purple}\or \color{Turque}\or \color{Blue}\or
               \color{Magenta}\or \color{Gold}\or \color{Seaweed}\or
                \color{Brown}\or\color{grey1}\or\color{grey2}\or
                 \color{grey3}\else\color{grey4}\fi#2}}
\def\CBox#1#2{{\color{#1}\fbox{\color{black}#2}}}
\definecolor{Slate} {rgb}{0.00,0.45,0.55}
\def\Gr#1{{\color{Slate}#1}}
\def\GRN#1{{\color{Green}#1}}
\def\RED#1{{\color{Red}#1}}

%%%%%%%%%%% ADDING COLOR %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% Yangrui Add The Lines of Code
%%%%%% That Start Here
\usepackage[enableskew,vcentermath]{youngtab}
\let\TC=\textcolor
\definecolor{Hey}{rgb}{.9,.05,.4}
\definecolor{orange}{rgb}{1,.5,0}
\definecolor{plum}{rgb}{.4,0,.6}
\definecolor{R}{rgb}{1,0,0}
\definecolor{G}{rgb}{0.1,0.7,0}
\definecolor{B}{rgb}{0,0,1}
%
\long\def\CMTblu#1{\leavevmode\TC{blue}{\sf#1}}
\long\def\CMTgrn#1{\leavevmode\TC{green}{\sf#1}}
\long\def\CMTred#1{\leavevmode\TC{red}{\sf#1}}
\long\def\CMTorg#1{\leavevmode\TC{orange}{\sf#1}}
\long\def\CMTR#1{\leavevmode\TC{R}{\sf#1}}
\long\def\CMTG#1{\leavevmode\TC{G}{\sf#1}}
\long\def\CMTB#1{\leavevmode\TC{B}{\sf#1}}
%%%%% And End Here
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%----------------------------------------------------------------------------------------
% CODE INCLUSION CONFIGURATION
%----------------------------------------------------------------------------------------
\usepackage{lipsum}
\usepackage{listings}
\definecolor{MyDarkGreen}{rgb}{0.0,0.4,0.0} % This is the color used for comments
\lstloadlanguages{Perl} % Load Perl syntax for listings, for a list of other languages supported see: ftp://ftp.tex.ac.uk/tex-archive/macros/latex/contrib/listings/listings.pdf
\lstset{language=Perl, % Use Perl in this example
        frame=single, % Single frame around code
        basicstyle=\small\ttfamily, % Use small true type font
        keywordstyle=[1]\color{Blue}\bf, % Perl functions bold and blue
        keywordstyle=[2]\color{Purple}, % Perl function arguments purple
        keywordstyle=[3]\color{Blue}\underbar, % Custom functions underlined and blue
        identifierstyle=, % Nothing special about identifiers                                         
        commentstyle=\usefont{T1}{pcr}{m}{sl}\color{MyDarkGreen}\small, % Comments small dark green courier font
        stringstyle=\color{Purple}, % Strings are purple
        showstringspaces=false, % Don't put marks in string spaces
        tabsize=5, % 5 spaces per tab
        %
        % Put standard Perl functions not included in the default language here
        morekeywords={rand},
        %
        % Put Perl function parameters here
        morekeywords=[2]{on, off, interp},
        %
        % Put user defined functions here
        morekeywords=[3]{test},
        %
        morecomment=[l][\color{Blue}]{...}, % Line continuation (...) like blue comment
        numbers=left, % Line numbers on left
        firstnumber=1, % Line numbers start with line 1
        numberstyle=\tiny\color{Blue}, % Line numbers are blue and small
        stepnumber=5 % Line numbers go in steps of 5
}

% Creates a new command to include a perl script, the first parameter is the filename of the script (without .pl), the second parameter is the caption
\newcommand{\perlscript}[2]{
\begin{itemize}
\item[]\lstinputlisting[caption=#2,label=#1]{#1.pl}
\end{itemize}
}



%:Abbrev's
% Upright letters
\def\rD{{\rm D}}
\def\rI{{\rm I}}
\def\rJ{{\rm J}}
\def\rK{{\rm K}}
\def\rL{{\rm L}}
\def\rR{{\rm R}}

% hatted indices
\def\hi{{\hat\imath}}
\def\hj{{\hat\jmath}}
\def\hk{{\hat{k}}}
\def\hl{{\hat\ell}}
\def\MNote#1{{\color{red}$^{!\!!}$\marginpar{\raggedright\color{red}\tiny#1}}\ignorespaces}

\def\strk#1{\setbox0=\hbox{#1}\rlap{{\color{Red}\rule[1pt]{\wd0}{1mm}}}{#1}}


\def\fracm#1#2{\hbox{\large{${\frac{{#1}}{{#2}}}$}}}

\def\vCent#1{\vcenter{\hbox{\hss#1\hss}}}
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\ena}{\end{eqnarray}}
\newcommand{\CN}{{\cal N}}

\def\bj#1{{}_{\rm #1}}                          % special subscript

\def\pp{{\mathchoice
            %{general format
               %[w] = length of horizontal bars
               %[t] = thickness of the lines
               %[h] = length of the vertical line
               %[s] = spacing around the symbol
              %
              %\kern [s] pt%
              %\raise 1pt
              %\vbox{\hrule width [w] pt height [t] pt depth0pt
              %      \kern -([h]/3) pt
              %      \hbox{\kern ([w]-[t])/2 pt
              %            \vrule width [t] pt height [h] pt depth0pt
              %            }
              %      \kern -([h]/3) pt
              %      \hrule width [w] pt height [t] pt depth0pt}%
              %      \kern [s] pt
          {%displaystyle
              \kern 1pt%
              \raise 1pt
              \vbox{\hrule width5pt height0.4pt depth0pt
                    \kern -2pt
                    \hbox{\kern 2.3pt
                          \vrule width0.4pt height6pt depth0pt
                          }
                    \kern -2pt
                    \hrule width5pt height0.4pt depth0pt}%
                    \kern 1pt
           }
            {%textstyle
              \kern 1pt%
              \raise 1pt
              \vbox{\hrule width4.3pt height0.4pt depth0pt
                    \kern -1.8pt
                    \hbox{\kern 1.95pt
                          \vrule width0.4pt height5.4pt depth0pt
                          }
                    \kern -1.8pt
                    \hrule width4.3pt height0.4pt depth0pt}%
                    \kern 1pt
            }
            {%scriptstyle
              \kern 0.5pt%
              \raise 1pt
              \vbox{\hrule width4.0pt height0.3pt depth0pt
                    \kern -1.9pt  %[e]=0.15pt
                    \hbox{\kern 1.85pt
                          \vrule width0.3pt height5.7pt depth0pt
                          }
                    \kern -1.9pt
                    \hrule width4.0pt height0.3pt depth0pt}%
                    \kern 0.5pt
            }
            {%scriptscriptstyle
              \kern 0.5pt%
              \raise 1pt
              \vbox{\hrule width3.6pt height0.3pt depth0pt
                    \kern -1.5pt
                    \hbox{\kern 1.65pt
                          \vrule width0.3pt height4.5pt depth0pt
                          }
                    \kern -1.5pt
                    \hrule width3.6pt height0.3pt depth0pt}%
                    \kern 0.5pt%}
            }
        }}

\def\mm{{\mathchoice
                      %{general format %[w] = length of bars
                                       %[t] = thickness of bars
                                       %[g] = gap between bars
                                       %[s] = space around symbol
   %[w], [t], [s], [h]=3([g]) are taken from corresponding definitions of \pp
   %
                      %       \kern [s] pt
               %\raise 1pt    \vbox{\hrule width [w] pt height [t] pt depth0pt
               %                   \kern [g] pt
               %                   \hrule width [w] pt height[t] depth0pt}
               %              \kern [s] pt}
                  %
                       {%displaystyle
                             \kern 1pt
               \raise 1pt    \vbox{\hrule width5pt height0.4pt depth0pt
                                  \kern 2pt
                                  \hrule width5pt height0.4pt depth0pt}
                             \kern 1pt}
                       {%textstyle
                            \kern 1pt
               \raise 1pt \vbox{\hrule width4.3pt height0.4pt depth0pt
                                  \kern 1.8pt
                                  \hrule width4.3pt height0.4pt depth0pt}
                             \kern 1pt}
                       {%scriptstyle
                            \kern 0.5pt
               \raise 1pt
                            \vbox{\hrule width4.0pt height0.3pt depth0pt
                                  \kern 1.9pt
                                  \hrule width4.0pt height0.3pt depth0pt}
                            \kern 1pt}
                       {%scriptscriptstyle
                           \kern 0.5pt
             \raise 1pt  \vbox{\hrule width3.6pt height0.3pt depth0pt
                                  \kern 1.5pt
                                  \hrule width3.6pt height0.3pt depth0pt}
                           \kern 0.5pt}
                       }}

\def\ad{{\kern0.5pt
                   \alpha \kern-5.05pt \raise5.8pt\hbox{$\textstyle.$}\kern
0.5pt}}

\def\bd{{\kern0.5pt
                   \beta \kern-5.05pt \raise5.8pt\hbox{$\textstyle.$}\kern
0.5pt}}


\def\qd{{\kern0.5pt
                   q \kern-5.05pt \raise5.8pt\hbox{$\textstyle.$}\kern
0.5pt}}
\def\Dot#1{{\kern0.5pt
     {#1} \kern-5.05pt \raise5.8pt\hbox{$\textstyle.$}\kern
0.5pt}}


%:Underline for text or math

\catcode`@=11
\def\un#1{\relax\ifmmode\@@underline#1\else
        $\@@underline{\hbox{#1}}$\relax\fi}
\catcode`@=12

%:Accents and foreign (in text):

\let\under=\b                   % bar-under (but see \un above)
\let\ced=\c                     % cedilla
\let\du=\d                      % dot-under
\let\um=\H                      % Hungarian umlaut
\let\sll=\l                     % slashed (suppressed) l (Polish)
\let\Sll=\L                     % " L
\let\slo=\o                     % slashed o (Scandinavian)
\let\Slo=\O                     % " O
\let\tie=\t                     % tie-after (semicircle connecting two letters)
\let\br=\u                      % breve
                % Also: \`        grave
                %       \'        acute
                %       \v        hacek (check)
                %       \^        circumflex (hat)
                %       \~        tilde (squiggle)
                %       \=        macron (bar-over)
                %       \.        dot (over)
                %       \"        umlaut (dieresis)
                %       \aa \AA   A-with-circle (Scandinavian)
                %       \ae \AE   ligature (Latin & Scandinavian)
                %       \oe \OE   " (French)
                %       \ss       es-zet (German sharp s)
                %       \$  \#  \&  \%  \pounds  {\it\&}  \Dots

%:Abbreviations for Greek letters

\def\a{\alpha}
\def\b{\beta}
\def\c{\chi}
\def\d{\delta}
\def\e{\epsilon}
\def\f{\phi}
\def\g{\gamma}
\def\h{\eta}
\def\i{\iota}
\def\j{\psi}
\def\k{\kappa}
\def\l{\lambda}
\def\m{\mu}
\def\n{\nu}
\def\o{\omega}
\def\p{\pi}
\def\q{\theta}
\def\r{\rho}
\def\s{\sigma}
\def\t{\tau}
\def\u{\upsilon}
\def\x{\xi}
\def\z{\zeta}
\def\D{\Delta}
\def\F{\Phi}
\def\G{\Gamma}
\def\J{\Psi}
\def\L{\Lambda}
\def\O{\Omega}
\def\P{\Pi}
\def\Q{\Theta}
\def\S{\Sigma}
\def\U{\Upsilon}
\def\X{\Xi}

%:Calligraphic letters

\def\ca{{\cal A}}
\def\cb{{\cal B}}
\def\cc{{\cal S}}
\def\cd{{\cal D}}
\def\ce{{\cal E}}
\def\cf{{\cal F}}
\def\cg{{\cal G}}
\def\ch{{\cal H}}
\def\ci{{\cal I}}
\def\cj{{\cal J}}
\def\ck{{\cal K}}
\def\cl{{\cal L}}
\def\cm{{\cal M}}
\def\cn{{\cal N}}
\def\co{{\cal O}}
\def\cp{{\cal P}}
\def\cq{{\cal Q}}
\def\car{{\cal R}}
\def\cs{{\cal P}}
\def\ct{{\cal T}}
\def\cu{{\cal U}}
\def\cv{{\cal V}}
\def\cw{{\cal W}}
\def\cx{{\cal X}}
\def\cy{{\cal Y}}
\def\cz{{\cal Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% Definition for a slash over a letter
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
%:from M. Peskin
\def\dslash{\not{\hbox{\kern-2pt $\partial$}}}
\def\Dslash{\not{\hbox{\kern-4pt $D$}}}
\def\pslash{\not{\hbox{\kern-2.3pt $p$}}}
%
%
 \newtoks\slashfraction
 \slashfraction={.13}
 \def\slash#1{\setbox0\hbox{$ #1 $}
 \setbox0\hbox to \the\slashfraction\wd0{\hss \box0}/\box0 }
 
% EXAMPLE OF HOW TO USE IT
% $\slash D$
% {\slashfraction={.075} $\slash{\cal A}$}
% $\slash B$
% $\slash a$
% {\slashfraction={.09} $\slash p$}
% $\slash q$
 
%:Fonts

\def\Go#1{{\hbox{\go #1}}}      % Gothic for single characters in equations
\def\Sc#1{{\hbox{\sc #1}}}      % script for single characters in equations
\def\Sf#1{{\hbox{\sf #1}}}      % sans serif for single characters in equations
\font\ro=cmsy10                          % font with rope
\def\kcl{{\hbox{\ro \char'170}}}        % left-handed rope
\def\kcr{{\hbox{\ro \char'170}}}                % right-handed rope
\def\ktl{{\hbox{\ro \char'170}}}        % top end for left-handed rope
\def\ktr{{\hbox{\ro \char'170}}}        % " right
\def\kbl{{\hbox{\ro \char'170}}}        % " bottom left
\def\kbr{{\hbox{\ro \char'170}}}        % " right
                        % Also:  \rm      Roman (default for text)
                        %        \bf      boldface
                        %        \it      italic
                        %        \mit     math italic (default for equations)
                        %        \sl      slanted
                        %        \em      emphatic
                        %        \tt      typewriter
                        % and sizes:    \tiny
                        %               \scriptsize
                        %               \footnotesize
                        %               \small
                        %               \normalsize
                        %               \large
                        %               \Large
                        %               \LARGE
                        %               \huge
                        %               \Huge

%:Math symbols

\def\ip{{=\!\!\! \mid}}                                    % 2-d plus
                                                        %vector index

\def\plpl{\raise-2pt\hbox{$\raise3pt\hbox{$_+$}\hskip-6.67pt\raise0.0pt
\hbox{$^+$}\hskip 0.01pt$}}
\def\mimi{\raise-2pt\hbox{$\raise3pt\hbox{$_-$}\hskip-6.67pt\raise0.0pt
\hbox{$^-$}\hskip 0.01pt$}}

\def\bo{{\raise.15ex\hbox{\large$\Box$}}}               % D'Alembertian
\def\cbo{\Sc [}                                         % curly "
\def\pa{\partial}                                       % curly d
\def\de{\nabla}                                         % del
\def\dell{\bigtriangledown}                             % hi ho the dairy-o
\def\su{\sum}                                           % summation
\def\pr{\prod}                                          % product
\def\iff{\leftrightarrow}                               % <-->
\def\conj{{\hbox{\large *}}}                            % complex conjugate
\def\ltap{\raisebox{-.4ex}{\rlap{$\sim$}} \raisebox{.4ex}{$<$}}   % < or ~
\def\gtap{\raisebox{-.4ex}{\rlap{$\sim$}} \raisebox{.4ex}{$>$}}   % > or ~
\def\TH{{\raise.2ex\hbox{$\displaystyle \bigodot$}\mskip-4.7mu \llap H \;}}
\def\face{{\raise.2ex\hbox{$\displaystyle \bigodot$}\mskip-2.2mu \llap {$\ddot
        \smile$}}}                                      % happy face
\def\dg{\sp\dagger}                                     % hermitian conjugate
\def\ddg{\sp\ddagger}                                   % double dagger
                        % Also:  \int  \oint              integral, contour
                        %        \hbar                    h bar
                        %        \infty                   infinity
                        %        \sqrt                    square root
                        %        \pm  \mp                 plus or minus
                        %        \cdot  \cdots            centered dot(s)
                        %        \oplus  \otimes          group theory
                        %        \equiv                   equivalence
                        %        \sim                     ~
                        %        \approx                  approximately =
                        %        \propto                  funny alpha
                        %        \ne                      not =
                        %        \le \ge                  < or = , > or =
                        %        \{  \}                   braces
                        %        \to  \gets               -> , <-
                        % and spaces:  \,  \:  \;  \quad  \qquad
                        %              \!                 (negative)


\font\tenex=cmex10 scaled 1200

\def\dt#1{\on{\hbox{\bf .}}{#1}}                % (big) dot over
\def\Dot#1{\dt{#1}}


\def\gfrac#1#2{\frac {\scriptstyle{#1}}
        {\mbox{\raisebox{-.6ex}{$\scriptstyle{#2}$}}}}
\def\gg{{\hbox{\sc g}}}


%:Math stuff with one argument

\def\sp#1{{}^{#1}}                              % superscript (unaligned)
\def\sb#1{{}_{#1}}                              % sub"
\def\oldsl#1{\rlap/#1}                          % poor slash
\def\sl#1{\rlap{\hbox{$\mskip 1 mu /$}}#1}      % good slash for lower case
\def\Sl#1{\rlap{\hbox{$\mskip 3 mu /$}}#1}      % " upper
\def\SL#1{\rlap{\hbox{$\mskip 4.5 mu /$}}#1}    % " fat stuff (e.g., M)
\def\PMMM#1{\rlap{\hbox{$\mskip 2 mu | $}}#1}   %
\def\PMM#1{\rlap{\hbox{$\mskip 4 mu ~ \mid $}}#1}       %
\def\Tilde#1{\widetilde{#1}}                    % big tilde
\def\Hat#1{\widehat{#1}}                        % big hat
\def\Bar#1{\overline{#1}}                       % big bar
\def\bra#1{\left\langle #1\right|}              % < |
\def\ket#1{\left| #1\right\rangle}              % | >
\def\VEV#1{\left\langle #1\right\rangle}        % < >
\def\abs#1{\left| #1\right|}                    % | |
\def\leftrightarrowfill{$\mathsurround=0pt \mathord\leftarrow \mkern-6mu
        \cleaders\hbox{$\mkern-2mu \mathord- \mkern-2mu$}\hfill
        \mkern-6mu \mathord\rightarrow$}
\def\dvec#1{\vbox{\ialign{##\crcr
        \leftrightarrowfill\crcr\noalign{\kern-1pt\nointerlineskip}
        $\hfil\displaystyle{#1}\hfil$\crcr}}}           % <--> accent
\def\dt#1{{\buildrel {\hbox{\LARGE .}} \over {#1}}}     % dot-over for sp/sb
\def\dtt#1{{\buildrel \bullet \over {#1}}}              % alternate "
\def\der#1{{\pa \over \pa {#1}}}                % partial derivative
\def\fder#1{{\d \over \d {#1}}}                 % functional derivative
                % Also math accents:    \bar
                %                       \check
                %                       \hat
                %                       \tilde
                %                       \acute
                %                       \grave
                %                       \breve
                %                       \Dot    (over)
                %                       \ddot   (umlaut)
                %                       \vec    (vector)

%:Math stuff with more than one argument

\def\fracm#1#2{\hbox{\large{${\frac{{#1}}{{#2}}}$}}}
\def\ha{\frac12}                                        % 1/2
\def\sfrac#1#2{{\vphantom1\smash{\lower.5ex\hbox{\small$#1$}}\over
        \vphantom1\smash{\raise.4ex\hbox{\small$#2$}}}} % alternate fraction
\def\bfrac#1#2{{\vphantom1\smash{\lower.5ex\hbox{$#1$}}\over
        \vphantom1\smash{\raise.3ex\hbox{$#2$}}}}       % "
\def\afrac#1#2{{\vphantom1\smash{\lower.5ex\hbox{$#1$}}\over#2}}    % "
\def\partder#1#2{{\partial #1\over\partial #2}}   % partial derivative of
\def\parvar#1#2{{\d #1\over \d #2}}               % variation of
\def\secder#1#2#3{{\partial^2 #1\over\partial #2 \partial #3}}  % second "
\def\on#1#2{\mathop{\null#2}\limits^{#1}}               % arbitrary accent
\def\bvec#1{\on\leftarrow{#1}}                  % backward vector accent
\def\oover#1{\on\circ{#1}}                              % circle accent



%%%%%%%%%%%%%%%%%%%%%% new definitions %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% operators %%%%%%%%%%%%%%%%%%%%%%
\def\opC{{\bm{\cal S}}}
\def\opCb{{\bm {\Bar{\cal S}}}}
\def\opN{{\bm{\cal N}}}
\def\opNb{{\bm {\Bar{\cal N}}}}
\def\opA{{\bm{\cal A}}}
\def\opAb{{\bm {\Bar{\cal A}}}}
\def\opR{{\bm{\cal R}}}
\def\opBox{{\bm {{}_\bo}}}
\def\opDeltaM{{\bm \Delta ^-}}
\def\opDeltaP{{\bm \Delta ^+}}
\def\opDelta{{\bm \Delta }}
\def\opDeltaT{{\bm {\tilde \Delta}}}
\def\opDsq{D^2}
\def\opDbsq{{\Bar D}^2}
%%%%%%%%%%%%%%%%%%%%%%%% kets %%%%%%%%%%%%%%%%%%%%%%%%
\def\ketT{|{\bm T}\rangle}
\def\ketTb{|\Bar{ {\bm T}}\rangle}
\def\ketG{|{\bm G}\rangle}
\def\ketGb{|\Bar{ {\bm G}}\rangle}
\def\ketK{|{\bm K}\rangle}
\def\ketKb{|\Bar{ {\bm K}}\rangle}
\def\ketH{|{\bm H}\rangle}
\def\ketW{|{\bm W}\rangle}
\def\ketW{|{\bm W}\rangle}
\def\ketUp{|{\bm {\Upsilon} }\rangle}
\def\ketUb{|\Bar{ {\bm U}}\rangle}
\def\ketV{|{\bm V}\rangle}
\def\ketL{|{\bm L}\rangle}
\def\ketLb{|\Bar{ {\bm L}}\rangle}
\def\ketKO{|{\bm K_1}\rangle}
\def\ketKT{|{\bm K_2}\rangle}
\def\ketKib{|\Bar{ {\bm K_i}}\rangle}
\def\ketKi{|{\bm K_i}\rangle}
\def\ketEperp{|{\bm E ^ \perp}\rangle}
\def\ketEpar{|{\bm E ^ \parallel}\rangle}
\def\ketGamma{|{\bm \Gamma }\rangle}
\def\ketGammab{|{\bm {\Bar \Gamma }}\rangle}
\def\ketUpsilonb{|{\bm {\Bar \Upsilon }}\rangle}
\def\ketPsi{|{\bm  \Psi }\rangle}
\def\ketPsib{|{\bm {\Bar \Psi }}\rangle}
\def\ketPhi{|{\bm  \Phi }\rangle}
\def\ketPhib{|{\bm {\Bar \Phi }}\rangle}
\def\ketLambda{|{\bm  \Lambda }\rangle}
\def\ketLambdab{|{\bm {\Bar \Lambda }}\rangle}
\def\ketEta{|{\bm  \eta }\rangle}
\def\ketEtab{|{\bm {\Bar \eta }}\rangle}
\def\ketSigma{|{\bm  \Sigma }\rangle}
\def\ketSigmab{|{\bm {\Bar \Sigma }}\rangle}
%%%%%%%%%%%%%%%%%%%%%%%%ets%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\etT{{\bm T}\rangle}
\def\etTb{\Bar{ {\bm T}}\rangle}
\def\etG{{\bm G}\rangle}
\def\etGb{\Bar{ {\bm G}}\rangle}
\def\etH{{\bm H}\rangle}
\def\etW{{\bm W}\rangle}
\def\etV{{\bm V}\rangle}
\def\etL{{\bm L}\rangle}
\def\etLb{\Bar{ {\bm L}}\rangle}
\def\etEperp{{\bm E ^ \perp}\rangle}
\def\etEpar{{\bm E ^ \parallel}\rangle}
\def\etGamma{{\bm \Gamma }\rangle}
\def\etGammab{{\bm {\Bar \Gamma }}\rangle}
\def\etPsi{{\bm  \Psi }\rangle}
\def\etPsib{{\bm {\Bar \Psi }}\rangle}
\def\etPhi{ {\bm \Phi }\rangle}
\def\etPhib{{\bm {\Bar \Phi }}\rangle}
\def\etEta{{\bm  \eta }\rangle}
\def\etEtab{{\bm {\Bar \eta }}\rangle}
%%%%%%%%%%%%%%%%%%%%%%%%bras%%%%%%%%%%%%%%%%%%%%%%%%%
\def\braH{\langle {\bm H}|}
\def\braL{\langle {\bm L}|}
\def\braW{\langle {\bm W}|}
\def\braGamma{\langle {\bm \Gamma}|}
\def\braGammab{\langle {\bm {\Bar \Gamma }}|}
\def\braGb{\langle {\bm {\Bar G }}|}
\def\braG{\langle {\bm G}|}
\def\braV{\langle {\bm V}|}
\def\braUb{\langle {\bm {\Bar U }}|}
\def\braU{\langle {\bm U}|}
\def\braPhi{\langle {\bm \Phi}|}
\def\braPhib{\langle {\bm {\Bar \Phi }}|}
\def\braPsi{\langle {\bm \Psi}|}
\def\braPsib{\langle {\bm {\Bar \Psi }}|}
\def\braSigma{\langle {\bm \Sigma}|}
\def\braSigmab{\langle {\bm {\Bar \Sigma }}|}
\def\braEta{\langle {\bm \eta}|}
\def\braEtab{\langle {\bm {\Bar \eta }}|}



\def\pa{\partial}      
\let\bm\relax
\newcommand{\bm}[1]{{\boldsymbol{#1}}}

\def\ad{{\Dot{\alpha}}}
\def\bd{{\Dot{\beta}}}
\def\Del{\nabla}
\def\Delb{\Bar{\nabla}}
\def\Delp{\nabla_{+}}
\def\Delm{\nabla_{-}}
\def\Delpd{\nabla_{\pd}}
\def\Delmd{\nabla_{\md}}
\def\Delpp{\nabla_{\pp}}
\def\Delmm{\nabla_{\mm}}
\def\Delsq{\nabla^2}
\def\Delbsq{{\Bar{\nabla}}^2}
\def\Dela{\nabla_{\alpha}}
\def\Delad{\nabla_{\Dot{\alpha}}}
\def\DelA{\nabla_A}
\def\Deltsq{{\Tilde{\Del}}^2}
\def\di{\pa}
\def\Dpd{{\rm D}_{\pd}}
\def\Dmd{{\rm D}_{\md}}
\def\Dpp{{\rm D}_{\pp}}
\def\Dmm{{\rm D}_{\mm}}
\def\Dpparl{\buildrel \leftrightarrow \over {\cal D}_{\pp}}
\def\Dmmarl{\buildrel \leftrightarrow \over {\cal D}_{\mm}}


%:Jim's border
 \font\rOpe=cmsy10                        % Ersatz for the non-standard rope font
 \def\kcl{{\hbox{\rOpe\char'170}}}        % left-handed rope
 \def\ktl{{\hbox{\rOpe\char'170}}}        % top end for left-handed rope
 \def\kbl{{\hbox{\rOpe\char'170}}}        % bottom end for left-handed rope
 %\reflectbox is defined in the "graphicx" package
 \def\kcr{{\reflectbox{\rOpe\char'170}}}        % right-handed rope
 \def\ktr{{\reflectbox{\rOpe\char'170}}}        % top end for right-handed rope
 \def\kbr{{\reflectbox{\rOpe\char'170}}}        % bottom end for right-handed rope
 \def\Border{\vbox{\hsize0pt% braided border
        \setlength{\unitlength}{1mm}
        \newcount\xco
        \newcount\yco
        \xco=-21
        \yco=12
        \begin{picture}(0,0)(-7.5,0)
        \put(\xco,\yco){$\ktl$}
        \advance\yco by-1
        {\loop
        \put(\xco,\yco){$\kcr$}
        \advance\yco by-2
        \ifnum\yco>-240
        \repeat
        \put(\xco,\yco){$\kbl$}}
        \xco=170
        \yco=12
        \put(\xco,\yco){$\ktr$}
        \advance\yco by-1
        {\loop
        \put(\xco,\yco){$\kcr$}
        \advance\yco by-2
        \ifnum\yco>-240
        \repeat
        \put(\xco,\yco){$\kbr$}}
        % \scalebox requires the "graphicx" package !
        \put(-19.5,13){\scalebox{.6065}{%
         University of Maryland Center for String and Particle  Theory \&\ Physics Department%
        |University of Maryland Center for String and Particle  Theory \&\ Physics Department}}
        \put(-19.5,-241.5){\scalebox{.5835}{%
         ****University of Maryland * Center for String and
         Particle  Theory* Physics Department****University of Maryland *Center
        for String and Particle  Theory* Physics Department}}
        \end{picture}
        \par\vskip-8mm}}
\definecolor{UMred}{rgb}{.9,.05,.2}
\definecolor{HUblue}{rgb}{.0,.3,.7}
 \def\UMbanner{\vbox{\hsize0pt% The "UM" banner
        \setlength{\unitlength}{.4mm}
        \thicklines  
        \begin{picture}(0,0)(-30,-10)
        \put(165,2){\line(1,0){4}}
        \put(170,2){\line(1,0){4}}
        \put(180,2){\line(1,0){4}}
        \put(175,-14){\line(1,0){4}}
        \put(180,-14){\line(1,0){4}}
        \put(185,-14){\line(1,0){4}}
        \put(169,-14){\line(0,1){16}}
        \put(170,-14){\line(0,1){16}}
        \put(179,-14){\line(0,1){16}}
        \put(180,-14){\line(0,1){16}}
        \put(184,-14){\line(0,1){16}}
        \put(185,-14){\line(0,1){16}}
        \put(169,2){\oval(8,32)[bl]}
        \put(170,2){\oval(8,32)[br]}
        \put(179,-14){\oval(8,32)[tl]}
        \put(185,-14){\oval(8,32)[tr]}
        \end{picture}
        \par\vskip-6.5mm
        \thicklines}}


%:Coloring
\definecolor{Red}    {rgb}{0.90,0.00,0.12} %  1
\definecolor{Blue}   {rgb}{0.00,0.00,1.00} %  2
\definecolor{Green}  {rgb}{0.10,0.70,0.10} %  3
\definecolor{Turque} {rgb}{0.00,0.65,0.85} %  4
\definecolor{Orange} {rgb}{1.00,0.50,0.15} %  5
\definecolor{Magenta}{rgb}{1.00,0.00,1.00} %  6
\definecolor{Gold}   {rgb}{1.00,0.75,0.25} %  7
\definecolor{Seaweed}{rgb}{0.01,0.24,0.09} %  8
\definecolor{Purple} {rgb}{0.50,0.25,0.55} %  9
\definecolor{Brown}  {rgb}{0.43,0.26,0.32} % 10
\definecolor{grey1}  {rgb}{0.20,0.20,0.20} % 11
\definecolor{grey2}  {rgb}{0.40,0.40,0.40} % 12
\definecolor{grey3}  {rgb}{0.60,0.60,0.60} % 13
\definecolor{grey4}  {rgb}{0.80,0.80,0.80} % 14
\definecolor{grey5}  {rgb}{0.90,0.90,0.90} % 15
\def\C#1#2{{\ifcase#1\or%TH color scheme
             \color{Red}\or \color{Green}\or \color{Blue}\or\
              \color{Turque}\or \color{Orange}\or \color{Magenta}\or
               \color{Gold}\or \color{Seaweed}\or \color{Purple}\or
                \color{Brown}\or\color{grey1}\or\color{grey2}\or
                 \color{grey3}\else\color{grey4}\fi#2}}
\def\CBox#1#2{{\color{#1}\fbox{\color{black}#2}}}
\definecolor{Slate} {rgb}{0.00,0.45,0.55}
\def\Gr#1{{\color{Slate}#1}}

%:Jim's footnote style
\def\Ft#1{\,\footnote{#1}}
\newdimen\parshift\parshift=\parindent
\catcode`@=11
 \long\def\@footnotetext#1{\insert\footins{\reset@font\footnotesize
           \interlinepenalty\interfootnotelinepenalty\splittopskip%
            \footnotesep\splitmaxdepth\dp\strutbox\floatingpenalty\@MM%
             \hsize\columnwidth\addtolength{\hsize}{-2\parindent}
              \@parboxrestore\protected@edef\@currentlabel%
              {\csname p@footnote\endcsname\@thefnmark}%
                \color@begingroup%
                 \@makefntext{\rule\z@\footnotesep\ignorespaces#1%
                  \@finalstrut\strutbox}%
                \color@endgroup}}
 \long\def\@makefntext#1{\hglue\parshift%
           \vbox{\noindent\baselineskip=11pt plus.5pt minus.5pt\hb@xt@0em{\hss\@makefnmark\kern1pt}#1}}
%\show\footnote
\catcode`@=12


%:Aligned equations

\newskip\humongous \humongous=0pt plus 1000pt minus 1000pt
\def\caja{\mathsurround=0pt}
\def\eqalign#1{\,\vcenter{\openup2\jot \caja
        \ialign{\strut \hfil$\displaystyle{##}$&$
        \displaystyle{{}##}$\hfil\crcr#1\crcr}}\,}
\newif\ifdtup
\def\panorama{\global\dtuptrue \openup2\jot \caja
        \everycr{\noalign{\ifdtup \global\dtupfalse
        \vskip-\lineskiplimit \vskip\normallineskiplimit
        \else \penalty\interdisplaylinepenalty \fi}}}
\def\eqalignno#1{\panorama Tabskip=\humongous                  % eqalignno
        \halign to\displaywidth{\hfil$\displaystyle{##}$
        Tabskip=0pt&$\displaystyle{{}##}$\hfil
        Tabskip=\humongous&\llap{$##$}Tabskip=0pt
        \crcr#1\crcr}}
\def\eqalignnotwo#1{\panorama Tabskip=\humongous
        \halign to\displaywidth{\hfil$\displaystyle{##}$
        Tabskip=0pt&$\displaystyle{{}##}$
        Tabskip=0pt&$\displaystyle{{}##}$\hfil
        Tabskip=\humongous&\llap{$##$}Tabskip=0pt
        \crcr#1\crcr}}

%:section-headings with after-indent
\makeatletter
\def\section{\@startsection{section}{1}{\z@}
        {3ex plus-1ex minus-.2ex}{1pt plus1pt}{\large\sf\bfseries\boldmath}}
\def\subsection{\@startsection{subsection}{2}{\z@}
         {1.5ex plus-1ex minus-.2ex}{0.01pt plus1pt}{\sf\slshape}}
\def\subsubsection{\@startsection{subsubsection}{3}{\z@}
          {1.5ex plus-1ex minus-.2ex}{0.01pt plus0.2pt}{\sf\boldmath}}
\def\paragraph{\@startsection{paragraph}{4}{\z@}
           {.75ex \@plus.5ex \@minus.2ex}{-2mm}{\sf\bfseries\boldmath}}
\makeatother

%:Options
%\usepackage[notcite,color]{showkeys}
 \allowdisplaybreaks
 \seceq

%H-DEFNs

\newcommand{\aone}{{\un a}_1}
\newcommand{\bone}{{\un b}_1}
\newcommand{\cone}{{\un c}_1}
\newcommand{\done}{{\un d}_1}
\newcommand{\eone}{{\un e}_1}

\newcommand{\atwo}{{\un a}_2}
\newcommand{\btwo}{{\un b}_2}
\newcommand{\ctwo}{{\un c}_2}
\newcommand{\dtwo}{{\un d}_2}
\newcommand{\etwo}{{\un e}_2}

\newcommand{\athree}{{\un a}_3}
\newcommand{\bthree}{{\un b}_3}
\newcommand{\cthree}{{\un c}_3}
\newcommand{\dthree}{{\un d}_3}
\newcommand{\ethree}{{\un e}_3}

\newcommand{\afour}{{\un a}_4}
\newcommand{\bfour}{{\un b}_4}
\newcommand{\cfour}{{\un c}_4}
\newcommand{\dfour}{{\un d}_4}
\newcommand{\efour}{{\un e}_4}

\newcommand{\afive}{{\un a}_5}
\newcommand{\bfive}{{\un b}_5}
\newcommand{\cfive}{{\un c}_5}
\newcommand{\dfive}{{\un d}_5}
\newcommand{\efive}{{\un e}_5}

\newcommand{\ap}{{\un a}_p}
\newcommand{\bq}{{\un b}_q}
\newcommand{\cunq}{{\un c}_q}
\newcommand{\fone}{{\un f}_1}
\newcommand{\gone}{{\un g}_1}
\newcommand{\hone}{{\un h}_1}
\newcommand{\ione}{{\un i}_1}
\newcommand{\jone}{{\un j}_1}
\newcommand{\kone}{{\un k}_1}
\newcommand{\lone}{{\un l}_1}
\newcommand{\mone}{\small{ {\un m}_1}}
\newcommand{\nnone}{{\un n}_1}
\newcommand{\oone}{{\un o}_1}
\newcommand{\dr}{{\un d}_r}
\newcommand{\er}{{\un e}_r}
\newcommand{\fr}{{\un f}_r}
\newcommand{\gs}{{\un g}_s}
\newcommand{\hs}{{\un h}_s}
\newcommand{\is}{{\un i}_s}
\newcommand{\js}{{\un j}_s}
\newcommand{\kt}{{\un k}_t}
\newcommand{\lt}{{\un l}_t}
\newcommand{\mt}{{\un m}_t}
\newcommand{\nt}{{\un n}_t}
\newcommand{\ot}{{\un o}_t}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Hazel New Commands %%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Tying rules
\newcommand{\dotline}{\,\,\,\bullet\hspace{-0.35em}-}
\newcommand{\linedot}{-\hspace{-0.35em}\bullet\,\,\,}

% Colors for tying rules
\definecolor{skyblue}{rgb}{0.12, 0.46, 1.00}
\definecolor{brightpink}{rgb}{1.0, 0.0, 0.5}
\definecolor{darkgreen}{rgb}{0.10, 0.75, 0.24}

% 3-column tying rules
\newcommand{\sym}{\color{skyblue}{\bm \circ}}
\newcommand{\antisym}{\color{brightpink}{\ast}}
\newcommand{\nosym}{\color{darkgreen}{\thicksim}}
\newcommand{\symone}{\color{skyblue}{1}}
\newcommand{\symtwo}{\color{skyblue}{2}}
\newcommand{\symthree}{\color{skyblue}{3}}
\newcommand{\nosymone}{\color{darkgreen}{1}}
\newcommand{\nosymtwo}{\color{darkgreen}{2}}
\newcommand{\nosymthree}{\color{darkgreen}{3}}
\newcommand{\antisymone}{\color{brightpink}{1}}
\newcommand{\antisymtwo}{\color{brightpink}{2}}
\newcommand{\antisymthree}{\color{brightpink}{3}}
\newcommand{\singleone}{\color{black}{1}}
\newcommand{\singletwo}{\color{black}{2}}
\newcommand{\singlethree}{\color{black}{3}}
\newcommand{\singlefour}{\color{black}{4}}

% 4-column tying rules
\newcommand{\dotlineup}{\raisebox{0.15em}{$\dotline$}}
\newcommand{\linedotup}{\raisebox{0.15em}{$\linedot$}}
\newcommand{\dotlinedown}{\raisebox{-0.15em}{$\dotline$}}
\newcommand{\linedotdown}{\raisebox{-0.15em}{$\linedot$}}
%
\newcommand{\dotlineupdot}{\raisebox{0.15em}{$\dotline$}\hspace{-1.35em}\raisebox{-0.15em}{$\cdots$}}
\newcommand{\linedotupdot}{\raisebox{0.15em}{$\linedot$}\hspace{-1.35em}\raisebox{-0.15em}{$\cdots$}}
\newcommand{\dotlinedowndot}{\raisebox{-0.15em}{$\dotline$}\hspace{-1.35em}\raisebox{0.15em}{$\cdots$}}
\newcommand{\linedotdowndot}{\raisebox{-0.15em}{$\linedot$}\hspace{-1.35em}\raisebox{0.15em}{$\cdots$}}
%
\newcommand{\dotlinebb}{\,\,\,{\color{skyblue}{\bullet}}\hspace{-0.35em}-}
\newcommand{\linedotbb}{-\hspace{-0.35em}{\color{skyblue}{\bullet}}\,\,\,}
%
\newcommand{\dotlineupbb}{\raisebox{0.15em}{$\dotlinebb$}}
\newcommand{\linedotupbb}{\raisebox{0.15em}{$\linedotbb$}}
\newcommand{\dotlinedownbb}{\raisebox{-0.15em}{$\dotlinebb$}}
\newcommand{\linedotdownbb}{\raisebox{-0.15em}{$\linedotbb$}}
%
\newcommand{\dotlineupdotbb}{\raisebox{0.15em}{$\dotlinebb$}\hspace{-1.35em}\raisebox{-0.15em}{$\cdots$}}
\newcommand{\linedotupdotbb}{\raisebox{0.15em}{$\linedotbb$}\hspace{-1.35em}\raisebox{-0.15em}{$\cdots$}}
\newcommand{\dotlinedowndotbb}{\raisebox{-0.15em}{$\dotlinebb$}\hspace{-1.35em}\raisebox{0.15em}{$\cdots$}}
\newcommand{\linedotdowndotbb}{\raisebox{-0.15em}{$\linedotbb$}\hspace{-1.35em}\raisebox{0.15em}{$\cdots$}}

% Bare ties
\newcommand{\tietie}{\CMTB{\hspace{-0.15em}\dotline\hspace{-0.6em}\linedot\hspace{-0.15em}}}

% Basic SYT
\newcommand{\sixteen}{{\raisebox{-0.1em}{$16$}}}
\newcommand{\sixteenbar}{{\raisebox{-0.1em}{$\overline{16}$}}}
%
\newcommand{\tinysixteen}{{\raisebox{-0.03em}{\scriptsize $16$}}}
\newcommand{\tinysixteenbar}{{\raisebox{-0.03em}{\scriptsize $\overline{16}$}}}
%
\newcommand{\indexsixteen}{\scalebox{.5}{$16$}}
\newcommand{\indexsixteenbar}{\scalebox{.5}{$\overline{16}$}}
%
\newcommand{\tinysixteenaltbar}{{\raisebox{-0.1em}{\tiny $\overset{(-)^{n}}{16~~}$}}}
\newcommand{\tinysixteenaltbarm}{{\raisebox{-0.1em}{\tiny $\overset{(-)^{m}}{16~~}$}}}
%
\newcommand{\SYTtri}{\mbox{\begin{picture}(4,4)
\put(1,0){\line(1,0){4}}
\put(1,0){\line(1,1){4}}
\put(5,0){\line(0,1){4}}
\end{picture}}}

% Arbitrary length YTs
\newcommand{\YThdots}[1]{\ydiagram{1}\ytableausetup{tabloids}\ydiagram[*(white) \cdots]{{#1}}\ytableausetup{notabloids}\ydiagram{1}}
\newcommand{\YTvdots}[1]{\renewcommand{\arraystretch}{0} \begin{tabular}{l} \ydiagram{1} \\ \ytableausetup{vtabloids}\ydiagram[*(white) \vdots]{#1}\ytableausetup{novtabloids} \\ \ydiagram{1} \end{tabular}}

% General BYT
\newcommand{\generalBYT}{{\CMTB{\ytableaushort{{}\cdots{}{}\cdots{}{}\cdots{}{}\cdots{}{
}\cdots{},{}\cdots{}{}\cdots{}{}\cdots{}{}\cdots{},{}\cdots{}{}\cdots{}{}\cdots{},{}\cdots{}{}\cdots{},{
}\cdots{}}}}}
%
\newcommand{\generalBYTpqrst}{{\overbrace{\CMTB{\ytableaushort{{}\cdots{},{}\cdots{},{
}\cdots{},{}\cdots{},{}\cdots{}}}}^{t} \hspace{-0.2em} \overbrace{\CMTB{\ytableaushort{{}\cdots{
},{}\cdots{},{}\cdots{},{}\cdots{},\none}}}^{s} \hspace{-0.2em} \overbrace{\CMTB{\ytableaushort{{
}\cdots{},{}\cdots{},{}\cdots{},\none,\none}}}^{r} \hspace{-0.2em} \overbrace{\CMTB{\ytableaushort{{
}\cdots{},{}\cdots{},\none,\none,\none}}}^{q} \hspace{-0.2em} \overbrace{\CMTB{\ytableaushort{{
}\cdots{},\none,\none,\none,\none}}}^{p}}}

% D-operator ``drop''
\newcommand{\drop}{\CMTB{\ytableaushort{\dotline{\none[-\hspace{-0.3em}\partial\,\,\,]}}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Modified D-operator
\newcommand{\Diop}{ \partial_{\ell} ~+~ i \, \ell \, \drop }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
